Meta-Auto-Decoder for Solving Parametric Partial Differential Equations

Many important problems in science and engineering require solving the so-called parametric partial differential equations (PDEs), i.e., PDEs with different physical parameters, boundary conditions, shapes of computation domains, etc. Recently, building learning-based numerical solvers for parametric PDEs has become an emerging new field. One category of methods such as the Deep Galerkin Method (DGM) and Physics-Informed Neural Networks (PINNs) aim to approximate the solution of the PDEs. They are typically unsupervised and mesh-free, but require going through the time-consuming network training process from scratch for each set of parameters of the PDE. Another category of methods such as Fourier Neural Operator (FNO) and Deep Operator Network (DeepONet) try to approximate the solution mapping directly. Being fast with only one forward inference for each PDE parameter without retraining, they often require a large corpus of paired input-output observations drawn from numerical simulations, and most of them need a predefined mesh as well. In this paper, we propose Meta-Auto-Decoder (MAD), a mesh-free and unsupervised deep learning method that enables the pre-trained model to be quickly adapted to equation instances by implicitly encoding (possibly heterogenous) PDE parameters as latent vectors. The proposed method MAD can be interpreted by manifold learning in infinite-dimensional spaces, granting it a geometric insight. Extensive numerical experiments show that the MAD method exhibits faster convergence speed without losing accuracy than other deep learning-based methods. The project page with code is available: https://gitee.com/mindspore/mindscience/tree/master/MindElec/.

==> sections/introduction.tex <==
\section{Introduction}\label{sec:intro}

\noindent
Many important problems in science and engineering, such as inverse problems, control and optimization, risk assessment, and uncertainty quantification \cite{cohen2015approximation,khoo2021solving}, require solving the so-called parametric PDEs, i.e., partial differential equations (PDEs) with different physical parameters, boundary conditions, or solution regions.
Mathematically, they require to solve the so-called \textit{parametric} PDEs that can be formally formulated as:
\begin{equation}\label{def:PDE}
	\begin{aligned}
		\mathcal{L}_x^\eta u &= \phi_\eta, \quad x \in \Omega \subset \R^d \\
		\mathcal{B}_x^\eta u &= 0, \qquad x \in \partial \Omega
	\end{aligned}
\end{equation}
where $\mathcal{L}^{\eta}$ and $\mathcal{B}^\eta$ are partial differential operators parametrized by $\eta$, and $x$ denotes the independent variable in spatiotemporal-dependent PDEs. 
Given $\mathcal{A} = \mathcal{A}(\Omega;\R^{d_{\eta}})$ and $\mathcal{U} = \mathcal{U}(\Omega;\R^{d_u})$, $\eta \in \mathcal{A}$ is the variable parameter of the PDEs and $u \in \mathcal{U}$ is the solution of the PDEs. Solving parametric PDEs requires to learn infinite-dimensional operator $G:\mathcal{A} \to \mathcal{U}$ that map any PDE parameter $\eta$ to its corresponding solution $u^\eta$ (i.e., the solution mapping).

% Traditional solvers, e.g., finite element methods (FEM) \cite{zienkiewicz1977finite} or finite difference methods (FDM) \cite{liszka1980finite}, may suffer from prohibitively long simulation time, which motivates the emerging new field of learning-based numerical solvers for parametric PDEs.

In recent years, learning-based PDE solvers have become very popular, and it is generally believed that learning-based PDE solvers have the potential to improve the solution speed \cite{raissi2018deep,ChiyuMaxJiang2020MeshfreeFlowNetAP,DmitriiKochkov2021MachineLA}.
The learning-based PDE solvers can be categorized into two categories in terms of the objects that are approximated by neural networks, i.e., the approximation of the solution $u^\eta$ and the approximation of the solution mapping $G$.
The methods \cite{raissi2018deep, sirignano2018dgm, weinan2018deep, zang2020weak} that directly approximate the solution of the PDEs are developed to solve fixed-parameter PDEs, where the loss functions are based on physical laws. These methods are typically unsupervised and mesh-free, making them flexible to use in practice. However, all these methods treat different PDE parameters as different tasks, and need to retrain a deep neural network from scratch for each task. When a large number of tasks with different PDE parameters need to be solved, these methods are computationally expensive and impractical.

The solution mapping approximation methods \cite{long2018pde,long2019pde,lu2019deeponet,bhattacharya2020model,li2020fourier} require only one forward inference for each PDE parameter $\eta$ without retraining.
Although these methods have demonstrated promising results across a wide range of applications, they require a large corpus of paired input-output observations that involve a large number of expensive numerical simulations. 
In addition, most of these methods \cite{long2018pde,long2019pde,bhattacharya2020model,li2020fourier} require a predefined mesh and utilize the labeled data on the mesh for training and inference. Although DeepONet \cite{lu2019deeponet} is mesh-free, it needs to explicitly encode heterogeneous PDE parameters, which is inconvenient to implement.

Recently, \citet{wang2021learning} proposed physics-informed DeepONet, which combines the respective advantages of PINNs and DeepONet, enabling DeepONet to learn the solution mapping without any labeled data and retraining.
However, physics-informed DeepONet has several problems as follows. 
First, it suffers from the same problem as DeepONet, namely that it is inconvenient to encode heterogeneous PDE parameters.
Second, it needs to collect a large number of training samples in the function space $\mathcal{A}$ to obtain an acceptable accuracy during inference. 
Finally, physics-informed is unable to work well with out-of-distribution (OOD) problems (i.e. PDE parameters for training and PDE parameters for inference are from different probability distributions).

In this paper, we propose Meta-Auto-Decoder (MAD), a mesh-free and unsupervised deep learning method that enables the pre-trained model to be quickly adapted to equation instances by implicitly encoding heterogenous PDE parameters as latent vectors.

The motivation of MAD is to hope that the model can have the following properties: label-free (unsupervised), mesh-free, fast transfer to new PDE parameters, auto-encoding of heterogeneous PDE parameters.
To achieve label-free and mesh-free goals, MAD can take advantage of physics-informed loss to train the neural network and use the spatiotemporal coordinates $x$ as part of the neural network input.
To achieve the fast transfer goals, we can view solving parametric PDEs as a meta-learning problem.
Different from conventional machine learning that learns to do a given task, meta-learning learns to improve the learning algorithm itself based on multiple learning episodes over a distribution of related tasks.
As a result, meta-learning can handle new tasks faster and better. 
Meta-MgNet \cite{2022Meta} is the first work that view solving parametric PDEs as a meta-learning problem, which is based on hypernet and the multigrid algorithm. Meta-MgNet can utilize the similarity between tasks to ensure fast transfer. 
[TODO:show the shortcoming of Meta-MgNet]. 
Different from Meta-MgNet, MAD learns a nonlinear approximation of the solution manifold from the perspective of manifold learning. When a new task comes, MAD achieves fast transfer by projecting the new task to the manifold and updating the manifold at the same time.
In order to facilitate the auto-encoding of heterogeneous PDE parameters, we use the auto-decoder architecture \cite{park2019deepsdf}, which implicitly encodes different PDE parameters into different latent vactors.



% Different from conventional machine learning that learns to do a given task, meta-learning learns to improve the learning algorithm itself based on multiple learning episodes over a distribution of related tasks. 
% As a result, meta-learning can handle new tasks faster and better. 
% Solving parametric PDEs can be treated as a meta-learning problem if considering that these PDEs share the same form of equations but only differ in parameters. 
% Recently \cite{liu2021novel} utilizes Reptile method to learn a good initial model that can be generalized across different tasks and finally accelerates unseen tasks. 
% We also try Reptile method to solve parametric PDEs but find that it may fail to improve convergence speed in some cases. 
% For example, little gain is achieved when use it to solve Maxwell's equations with variable coefficients (see Sec.\ref{sec:maxwell}).


% \cite{park2019deepsdf} present an interesting work in 3D computer vision that can generate any 3D shape from a shape description. 
% Each shape description is encoded as a latent vector, and an auto-decoder is constructed to represent the mapping from the latent space to a distribution of complex shapes. 
% We can consider it as a meta-learning work, and inspired by which we propose Meta-Auto-Decoder (MAD) that applies auto-decoder to solving parametric PDEs. 
% Parameter of an individual PDEs is encoded as a latent vector, and a deep neural network is pre-trained to represent the mapping from the parameter latent space to the solution space. 
% We extend the auto-decoder method in \cite{park2019deepsdf} by jointly fine-tuning the latent vector and the neural network to increase solution accuracy for unseen task, whereas the original auto-decoder method fine-tunes only latent vector.
% We further analyze and visually explain the mathematical principle behind our MAD method, which provides a deep insight on how and why MAD works from the perspective of manifold learning.


% Our proposed method has several advantages. 
% Firstly, as MAD uses physics-informed losses, it can work without any labeled data compared with neural operator methods. 
% Secondly, once the deep neural network is pre-trained, a new task can converge after only a few iterations without loss of accuracy, in contrast to neural approximation methods that must solve each task from scratch. 
% Thirdly, MAD exhibits more stable speed-up performance compared with other meta-learning method \cite{liu2021novel} and transfer learning method \cite{weinan2018deep}.

The main contributions of this paper are summarized as follows: 
\begin{itemize}
\item A mesh-free and label-free deep neural network approach is proposed to solve parametric PDEs. Based on meta-learning concept, once the neural network is pre-trained, solving a new task involves only a few iterations. In addition, the auto-decoder architecture adopted by MAD can realize auto-encoding of heterogeneous PDE parameters.
\item The mathematical intuition behind the MAD method is analyzed from the perspective of manifold learning. In short, a neural network is pre-trained to approximate the solution manifold, and the required solution is searched on the solution manifold or in a neighborhood of the solution manifold.
\item Extensive numerical experiments are carried out to demonstrate the effectiveness of our method, which show that MAD can significantly improve the convergence speed and has good extrapolation ability for OOD problems.
\end{itemize}

==> sections/methodology.tex <==
\section{Methodology}\label{sec:methodology}
In this section, we first review the physics-informed losses induced by parametric PDEs and then introduce our MAD method in detail.


\subsection{Physics-Informed Loss}
Given any PDE parameter $\eta\in\mathcal{A}$, we denote the physics-informed loss $L^\eta:\mathcal{U}\to[0,\infty)$ about Eq.\eqref{def:PDE} as
% \begin{equation}
% \begin{split}
% 	L^\eta[u] &= L_\text{r}^\eta[u] + \lambda_\text{bc}L_\text{bc}^\eta[u],\\
% 	L_\text{r}^\eta[u] &= \|\mathcal{L}_x^\eta u-\phi_\eta\|_{L^2(\Omega)}^2,\\
% 	L_\text{bc}^\eta[u] &= \|\mathcal{B}_x^\eta u\|_{L^2(\partial\Omega)}^2,
% \end{split}
% \end{equation}
\begin{equation}
\begin{split}
	L^\eta[u] = L_\text{r}^\eta[u] + \lambda_\text{bc}L_\text{bc}^\eta[u],
	\quad
	L_\text{r}^\eta[u] = \|\mathcal{L}_x^\eta u-\phi_\eta\|_{L^2(\Omega)}^2, \quad
	L_\text{bc}^\eta[u] = \|\mathcal{B}_x^\eta u\|_{L^2(\partial\Omega)}^2,
\end{split}
\end{equation}
where $L_\text{r}^\eta[u]$ and $L_\text{bc}^\eta[u]$ are the loss terms corresponding to PDE residual and boundary conditions (initial condition is taken as a special boundary condition), respectively.
$\lambda_\text{bc}>0$ is a weighting coefficient.
The solution mapping  
% \footnote{In the literature, we would call $G$ a ``solution operator" if $\mathcal{A}=\mathcal{A}(\Omega;\R^{d_\eta})$ is a separable Banach space of functions taking values in $\R^{d_\eta}$.
% A more general choice of $\mathcal{A}$ is allowed in this paper, for example a subset of some linear space, or a discrete set.} 
of Eq.\eqref{def:PDE} is defined as:
% \begin{equation}
% \begin{split}
% 	G:\mathcal{A}&\to\mathcal{U},\\
% 	\eta&\mapsto G(\eta)=u^\eta.
% \end{split}
% \end{equation}
\begin{equation}
\begin{split}
	G:\mathcal{A}&\to\mathcal{U},
	\; \eta\mapsto G(\eta)=u^\eta.
\end{split}
\end{equation}
To compute $G(\eta)$, i.e., getting the solution $u^\eta$ for given parameter $\eta\in\mathcal{A}$, the PINNs method \cite{raissi2019physics} tries 
to approximate $u^\eta(x)$ using a neural network $u(x;\theta)$, and find $\theta\in\Theta$ by solving the following optimization problem: 
\begin{equation}
	\argmin_\theta\hat L^\eta[u(x;\theta)],
\end{equation}
% where $\hat{L}^\eta[u]$ defines the Monte Carlo estimate of $L^\eta[u]$.
where
% \begin{equation}\label{eq:MCPIloss}
% 	\begin{split}
% 		\hat L^\eta[u]&=\hat L_\text{r}^\eta[u]+\lambda_\text{bc}\hat L_\text{bc}^\eta[u]
% 		\\&=\frac1{M_\text{r}}\sum_{j=1}^{M_\text{r}}\Bigl\|\mathcal{L}_x^\eta u(x_j^\text{r})-\phi_\eta(x_j^\text{r})\Bigr\|_2^2 +
% 		\\&\quad \frac{\lambda_\text{bc}}{M_\text{bc}}\sum_{j=1}^{M_\text{bc}}\Bigl\|\mathcal{B}_x^\eta u(x_j^\text{bc})\Bigr\|_2^2
% 	\end{split}
% \end{equation}
\vspace{-0.3cm}
\begin{equation}\label{eq:MCPIloss}
	\begin{split}
		\hat L^\eta[u]=\hat L_\text{r}^\eta[u]+\lambda_\text{bc}\hat L_\text{bc}^\eta[u]
		=\frac1{M_\text{r}}\sum_{j=1}^{M_\text{r}}\Bigl\|\mathcal{L}_x^\eta u(x_j^\text{r})-\phi_\eta(x_j^\text{r})\Bigr\|_2^2 +
		\frac{\lambda_\text{bc}}{M_\text{bc}}\sum_{j=1}^{M_\text{bc}}\Bigl\|\mathcal{B}_x^\eta u(x_j^\text{bc})\Bigr\|_2^2
	\end{split}
\end{equation}
is the Monte Carlo estimate of $L^\eta[u]$, and $\{x_j^\text{r}\}_{j\in\{1,\dots,M_\text{r}\}}$ and $\{x_j^\text{bc}\}_{j\in\{1,\dots,M_\text{bc}\}}$ are two sets of random sampling points in $\Omega$ and $\partial\Omega$, respectively. 
$M_\text{r}$ and $M_\text{bc}$ are the number of sampling points in $\Omega$ and $\partial \Omega$, respectively. 


\subsection{Meta-Auto-Decoder}\label{sec:MAD_L}

\begin{figure}
\begin{center}
\centerline{\includegraphics[width=0.7\columnwidth]{./figures/intro_AD.png}}
\caption{Schematic of Meta-Auto-Decoder.}
\label{fig:AD_DNN}
\end{center}
\end{figure}

To avoid training a specific neural network from scratch for each PDE parameter, we adopt meta-learning concept to realize fast solution of parametric PDEs. 
Our basic idea is firstly learning some universal meta-knowledge from a set of sampled tasks in the pre-training stage, and then solving a new task quickly by combining the task-specific knowledge with the shared meta-knowledge in the fine-tuning stage. 
To achieve auto-encoding of PDE parameters simultaneously, we also adapt the auto-decoder architecture in \cite{park2019deepsdf} to construct our parametric PDEs solver called Meta-Auto-Decoder (MAD), whose working principle is shown in Fig.\ref{fig:AD_DNN}. 
MAD implicitly encodes each PDE parameter $\eta$ into a latent vector $z$, and then concatenates the latent vector $z$ with the independent variable $x$ as the input of the neural network. 
The output $u$ of the neural network is the approximate solution and then physics-informed losses are obtained by automatic differentiation \cite{baydin2018automatic}.
In the pre-training stage, through minimizing the loss function, a pre-trained model parametrized by $\theta^*$ is learned for all tasks and each task is paired with its own decoded latent vector $z$.
Such a pre-trained model is considered as the meta knowledge as it is learned from the distribution of all tasks and the learned latent vector $z$ is the task-specific knowledge. 
When solving a new task in the fine-tuning stage, keep the model weight $\theta^*$ fixed and minimize the loss by fine-tuning $z$.
We formulate the problem of pre-training and fine-tuning as follows:

\paragraph{Pre-training Stage}
Given $N$ randomly generated PDE parameters $\eta_1,\dots,\eta_N\in\mathcal{A}$, we solve the following optimization problem
% \vspace{-0.3cm}
% \begin{equation}\label{eq:MADtr}
% 	\operatorname*{\arg\min}_{\theta,\{z_i\}_{i\in\{1,\dots,N\}}}\sum_{i=1}^{N}\left(\hat L^{\eta_i}[u(\cdot,z_i;\theta)]+\frac1{\sigma^2}\|z_i\|^2\right)
% \end{equation}
% to obtain the optimal model weight $\theta^*$ and corresponding latent vectors $\{z_i^*\}_{i\in\{1,\dots,N\}}$, where $\hat L^{\eta_i}$ is defined in~\eqref{eq:MCPIloss}.
\vspace{-0.3cm}
\begin{equation}\label{eq:MADtr}
	(\{z^*_i\}_{i\in\{1,\dots,N\}},\; \theta^*) = \operatorname*{\arg\min}_{\theta,\{z_i\}_{i\in\{1,\dots,N\}}}\sum_{i=1}^{N}\left(\hat L^{\eta_i}[u(\cdot,z_i;\theta)]+\frac1{\sigma^2}\|z_i\|^2\right),
\end{equation}
where $\theta^*$ is the optimal model weight and $\{z_i^*\}_{i\in\{1,\dots,N\}}$ are the optimal latent vectors for different PDE parameters, where $\hat L^{\eta_i}$ is defined in~\eqref{eq:MCPIloss}.
The regularization term $\frac1{\sigma^2}\|z_i\|^2$ is added for training stability.

\paragraph{Fine-tuning Stage}
Given a new PDE parameter $\eta_{\text{new}}$, we compute $G(\eta_{\text{new}})$ (i.e. find the solution $u^{\eta_{\text{new}}}$) as follows: 
keeping $\theta^*$ fixed, and minimize the following loss function to get
\begin{equation}\label{eq:MADinf}
	z_{\text{new}}^*=\operatorname*{\arg\min}_{z}\hat L^{\eta_{\text{new}}}[u(\cdot,z;\theta^*)]+\frac1{\sigma^2}\|z\|^2
,\end{equation}
then $u(\cdot,z_{\text{new}}^*;\theta^*)$ is the approximate solution of PDEs with parameter $\eta_{\text{new}}$.
To speed up convergence, we can set the initial value of $z$ to $z_i^*$ obtained in the pre-training stage whose PDE parameter $\eta_i$ is the nearest\footnote{We can discretize a function into a vector and then find the Euclidean distance between the two vectors as the distance between two PDE parameters.} to $\eta_{\text{new}}$.

% During the pre-training stage, our approach implicitly encodes each task by a trainable latent vector $z$. 
% % Different tasks share the same neural network backbone while the input is the concatenation of the latent vector $z$ and data points from each task. 
% Different tasks share the same neural network backbone while the input is the concatenation of the latent vector $z$ and data point $x$ from each task.
% Using physics-informed losses ($\mathcal{L}_x^\eta u - \Phi_\eta$ corresponds to the PDE residual and $\mathcal{B}_x^\eta u$ corresponds to the boundary condition), both the latent vector $z$ and model weight $\theta$ are updated during the pre-training stage.  
% To the end, a pre-trained model weight $\theta^*$ is learned for all tasks and each task is paired with its own decoded latent vector $z$. 
% Such pre-trained model weight $\theta^*$ is considered as the meta knowledge as it benefits from all tasks and the learned latent vector $z$ is the task-specific knowledge. 
% When dealing a new task, MAD only needs to fine-tune the new latent vector $z$.

\subsection{Manifold Learning Interpretation of MAD}

\begin{figure*}
\centering
\subfigure[Fine-tune $z$ only]{
	\label{fig:MAD}
	\includegraphics[width=0.42\columnwidth]{figures/method_ADintuition.png}
}
\subfigure[Fine-tune $z$ and $\theta$ simultaneously]{
	\label{fig:MADft}
	\includegraphics[width=0.42\columnwidth]{figures/method_ADintuition-ft.png}
}
\caption{
	Illustration of how MAD works from the manifold learning perspective.
}
\end{figure*}

% In order to reveal the mathematical principle behind the MAD method, 
We analyze the effectiveness of the MAD method from the manifold learning perspective.
Considering that parametric PDEs have similar equation forms and only differ in PDE parameters, we make the following assumption that we believe holds for at least some cases if not for all cases. 
\begin{assumption}\label{as:lowdim}
	The solution set $G(\mathcal{A})=\{G(\eta)\mid\eta\in\mathcal{A}\}\subset\mathcal{U}$ on a parameter set $\mathcal{A}$ is contained in a low-dimensional structure. 
	To be more specific, we assume that there is a finite-dimensional space $Z=\R^l$ (with $l\ll\dim\mathcal{U}$) and a Lipschitz continuous mapping
	$\bar G:Z\to\mathcal{U}$, such that $G(\mathcal{A})\subseteq\bar G(Z)$. 
	In other words, for any $\eta\in\mathcal{A}$,  $\exists$  $z\in Z$ satisfying $\bar G(z)=G(\eta)$. 
\end{assumption}

The mapping $\bar G$ is Lipschitz continuous if and only if there exists some $C>0$ such that $\bigl\|\bar G(z)-\bar G(z')\bigr\|_\mathcal{U}\le C\|z-z'\|$ for all $z,z'\in Z$. 
This Lipschitz continuous constraint excludes highly irregular mappings.
The assumption is obviously satisfied when $\mathcal{A}$ is a finite-dimensional space and $G$ is Lipschitz continuous (just take $Z=\mathcal{A}$, $\bar G=G$).
Since $\dim Z\ll\dim\mathcal{U}$ (the latter is usually infinity) holds, we may view the mapping $\bar G$ as some sort of ``decoder'', and $Z$ is the corresponding latent vector space, despite of the fact that there doesn't exist an ``encoder''.
With certain smoothness and non-degeneracy constraints on $\bar G$, $\bar G(Z)\subset\mathcal{U}$ forms an embedded submanifold, and therefore our MAD method can be viewed as a manifold-learning approach.

Once mapping $\bar G$ is learned as above, then for a given parameter $\eta$, we no longer need to search for the solution $u^\eta$ in the whole space $\mathcal{U}$. 
Instead, we may focus on the smaller subset $\bar G(Z)$, i.e. the class of functions in $\mathcal{U}$ that is parametrized by $Z$, since $u^\eta=G(\eta)\in\bar G(Z)$ holds for any $\eta\in\mathcal{A}$. 
We then solve the optimization problem
\begin{equation}
z^\eta=\operatorname*{\argmin}_{z}L^\eta[\bar G(z)],
\end{equation} 
\vskip -0.2in 
and $\bar G(z^\eta)$ is the approximate solution. 

Now assuming that the dimension of $Z$ is chosen (either empirically or through trial and error), we try to find the mapping $\bar G$. 
Since such a mapping is usually complex and hard to design by hand, we consider the $\theta$-parametrized version% G_\theta:Z\to\mathcal{U}
\footnote{For fixed $\theta$, the set $G_\theta(Z)$ is parametrized by $z\in Z$. 
When $\theta$ changes, this set changes accordingly. 
In some sense, $\theta$ parametrizes a parametrization. }
$G_\theta:Z\to\mathcal{U}$, and find the best $\theta$ automatically by solving an optimization problem. 
We use a neural network to represent $G_\theta$:
\begin{equation}
	G_\theta(z)(x)=f_\theta(x,z)
,\end{equation} 
where $f_\theta$ is a neural network whose input is the concatenation of $x\in\R^d$ and $z\in\R^l$. 

Subsequently, we can find the optimal network weight $\theta$ via training, with the target being $G(\mathcal{A})\subseteq G_\theta(Z)$. 
Assuming that the PDE parameters are generated from a probability distribution $\eta\sim p_\mathcal{A}$, then $G(\eta)\in G_\theta(Z)$ holds almost surely if and only if
% \begin{equation}\label{eq:l2dist}
% 	\begin{split}
% 	d(\theta) &=\operatorname*{\mathbb{E}}_{\eta\sim p_\mathcal{A}}\left[d_\mathcal{U}\bigl(u^\eta,G_\theta(Z)\bigr)\right]
% 			  \\&=\operatorname*{\mathbb{E}}_{\eta\sim p_\mathcal{A}}\left[\min_z\bigl\lVert u^\eta-f_\theta(\cdot,z)\bigr\rVert_\mathcal{U}\right] = 0,
% 	\end{split}
% \end{equation}
\vskip -0.2in 
\begin{equation}\label{eq:l2dist}
	\begin{split}
	d(\theta) =\operatorname*{\mathbb{E}}_{\eta\sim p_\mathcal{A}}\left[d_\mathcal{U}\bigl(u^\eta,G_\theta(Z)\bigr)\right]
			  =\operatorname*{\mathbb{E}}_{\eta\sim p_\mathcal{A}}\left[\min_z\bigl\lVert u^\eta-f_\theta(\cdot,z)\bigr\rVert_\mathcal{U}\right] = 0,
	\end{split}
\end{equation}
which suggests taking $\theta^* = \operatorname*{\arg\min}_{\theta} d(\theta)$. 
In case we do not have direct access to the exact solutions $u^\eta$, the equivalent condition
\begin{equation}
	d'(\theta)=\operatorname*{\mathbb{E}}_{\eta\sim p_\mathcal{A}}\left[\min_zL^\eta[f_\theta(\cdot,z)]\right] = 0
\end{equation}
is considered, and we minimize $d'(\theta)$ instead. 
In the specific implementation, the expectation on $\eta\sim p_\mathcal{A}$ is estimated by Monte Carlo samples $\eta_1,\dots,\eta_N$, and the optimal network weight $\theta$ is taken to be
\vspace{-0.3cm}
\begin{equation}\label{eq:rawMADtr}
	\theta^*\approx\operatorname*{\arg\min}_{\theta}\frac1N\sum_{i=1}^{N}\min_{z_i}L^{\eta_i}[f_\theta(\cdot,z_i)].
\end{equation}
\vspace{-0.2cm}
We further estimate the physics-informed loss $L^\eta$ using Monte Carlo method to obtain Eq.\ref{eq:MADtr}.

An intuitive illustration of how MAD works from the manifold learning perspective is given in Fig.\ref{fig:MAD}. 
The function space $\mathcal{U}$ is mapped to a 2-dimensional plane.
The blue solid curve represents the solution set $G(\mathcal{A})$ formed by exact solutions corresponding to all possible PDE parameters, and each point on the curve represents a exact solution corresponding to one PDE parameter.
The orange dotted curve represents the solution set $G_{\theta^*}(Z)$ obtained by the pre-trained model, and each point on the curve corresponds to a latent vector $z$.
Given a PDE parameter $\eta_{\text{new}} \in \mathcal{A}$, rather than searches in the entire function space $\mathcal{U}$, MAD only searches on the orange dotted curve to find an optimal $z$ such that its corresponding solution is nearest to the blue solid curve.

\subsection{A Visualization Example}\label{src:motivational_example}
\begin{figure*}
\centering
\subfigure[Pre-training]{
	\label{fig:MADtr}
	\includegraphics[width=0.5\columnwidth]{figures/method_demoAD_pretrain.png}
}
\subfigure[Fine-tuning]{
	\label{fig:MADinfL}
	\includegraphics[width=0.4\columnwidth]{figures/method_demoAD_finetune_l.png}
}
\caption{
Visualization of the MAD pre-training and fine-tuning process for the ODE problem.
}
\label{figs:MAD_example}
\end{figure*}

% In this subsection, we use an ordinary differential equation (ODE) to visualize the pre-training and fine-tuning processes of MAD.
% We take the problem domain to be $\Omega=(-\pi,\pi)\subset\R$, the set of variable ODE parameters $\mathcal{A}=\R$, and the latent space $Z=\R$. 
% For given $\eta\in\mathcal{A}$, the ODE
% \begin{align*}
% 	\frac{\mathrm{d}u}{\mathrm{d}x}&=\phi_\eta(x)=2(x-\eta)\cos\bigl((x-\eta)^2\bigr),
% 	\\u(\pm\pi)&=\sin\bigl((\pm\pi-\eta)^2\bigr)
% \end{align*}
% has a unique solution $u^\eta(x)=\sin\bigl((x-\eta)^2\bigr)$.
% We sample 20 points equidistantly on the interval $[0, 2]$ as variable ODE parameters, and randomly select one $\eta_{\text{new}}$ for fine-tuning stage and the rest $\{\eta_i\}_{i \in \{1,\cdots,19\}}$ for pre-training stage.

% In pre-training stage, MAD generates a sequence of $(\theta^{(m)}, \{z_i^{(m)}\}_{i\in\{1,\cdots,19\}})$ to train the neural network,
% 	and terminates at $m=200$ (enough for the neural network to learn the manifold) with the optimal $(\theta^*, \{z_i^*\}_{i\in\{1,\cdots,19\}})$.
% In order to visualize how the solution set $G_\theta(Z)$ evolves, we project the infinite-dimensional function space $\mathcal{U}=C([-\pi,\pi])$ onto a 2-dimensional plane using principal component analysis (PCA) method.
% Fig.\ref{fig:MADtr} visualizes how $G_\theta(Z)$ evolves and gradually fits $G(\mathcal{A})$ in pre-training stage.
% The set of exact solutions $G(\mathcal{A})$ forms a 1-dimensional manifold (i.e. the red solid curve), and the marked points $\{G(\eta_i)\}_{i \in \{1,\cdots,19\}}$ represent those ODE parameters $\{\eta_i\}_{i\in\{1,\cdots,19\}}$ used for pre-training.
% Each dotted curve represents a solution set $G_\theta^{(m)}(Z)$ obtained by the neural network at the $m$-th iteration with the points $G_{\theta^{(m)}}(z_i^{(m)})=f_{\theta^{(m)}}(\cdot,z_i^{(m)})$ also marked on the curve.
% As the number of iterations $m$ increases, the network weight $\theta=\theta^{(m)}$ updates, making the dotted curves evolve and finally fit the red solid curve, i.e., the target manifold $G(\mathcal{A})$.

% Fig.\ref{fig:MADinfL} illustrates the fine-tuning process for a given new ODE parameter $\eta_{\text{new}} \in \mathcal{A}$.
% As in Fig.\ref{fig:MADtr}, the red solid curve represents the set of exact solutions $G(\mathcal{A})$, while the cyan dotted curve represents the solution set $G_{\theta^*}(Z) = G_{\theta^{(200)}}(Z)$ obtained by the pre-trained network.
% As $z=z_{\text{new}}^{(m)}$ updates (i.e., through fine-tuning $z$), the marked point $G_{\theta^*}(z_{\text{new}}^{(m)})$ moves on the cyan dotted curve, and finally converges to the approximate solution $G_{\theta^*}(z_{\text{new}}^*) = G_{\theta^*}(z_{\text{new}}^{(12)}) \approx G(\eta_{\text{new}})$.


In this subsection, we use an ordinary differential equation (ODE) to visualize the pre-training and fine-tuning processes of MAD. Consider the following problem with domain $\Omega=(-\pi,\pi)\subset\R$:
\vspace{-0.2cm}
\begin{align*}
	\frac{\mathrm{d}u}{\mathrm{d}x}&=\phi_\eta(x)=2(x-\eta)\cos\bigl((x-\eta)^2\bigr),\qquad u(\pm\pi)=\sin\bigl((\pm\pi-\eta)^2\bigr).
\vspace{-0.3cm}
\end{align*}
We sample 20 points equidistantly on the interval $[0, 2]$ as variable ODE parameters, and randomly select one $\eta_{\text{new}}$ for fine-tuning stage and the rest $\{\eta_i\}_{i \in \{1,\cdots,19\}}$ for pre-training stage.
MAD generates a sequence of $(\theta^{(m)}, \{z_i^{(m)}\}_{i\in\{1,\cdots,19\}})$ in pre-training stage, and terminates at $m=200$ with the optimal $(\theta^*, \{z_i^*\}_{i\in\{1,\cdots,19\}})$.
We then project the infinite-dimensional function space $\mathcal{U}=C([-\pi,\pi])$ onto a 2-dimensional plane using Principal Component Algorithm (PCA).
Fig.\ref{fig:MADtr} visualizes how $G_\theta(Z)$ gradually fits $G(\mathcal{A})$ in pre-training stage.
The set of exact solutions $G(\mathcal{A})$ forms a 1-dimensional manifold (i.e. the red solid curve), and the marked points $\{G(\eta_i)\}_{i \in \{1,\cdots,19\}}$ represent corresponding ODE parameters used for pre-training.
Each dotted curve represents a solution set $G_\theta^{(m)}(Z)$ obtained by the neural network at the $m$-th iteration with the points $G_{\theta^{(m)}}(z_i^{(m)})=f_{\theta^{(m)}}(\cdot,z_i^{(m)})$ also marked on the curve.
As the number of iterations $m$ increases, the network weight $\theta=\theta^{(m)}$ updates, making the dotted curves evolve and finally fit the red solid curve, i.e., the target manifold $G(\mathcal{A})$.

Fig.\ref{fig:MADinfL} illustrates the fine-tuning process for a given new ODE parameter $\eta_{\text{new}} \in \mathcal{A}$.
As in Fig.\ref{fig:MADtr}, the red solid curve represents the set of exact solutions $G(\mathcal{A})$, while the cyan dotted curve represents the solution set $G_{\theta^*}(Z) = G_{\theta^{(200)}}(Z)$ obtained by the pre-trained network.
As $z=z_{\text{new}}^{(m)}$ updates (i.e., through fine-tuning $z$), the marked point $G_{\theta^*}(z_{\text{new}}^{(m)})$ moves on the cyan dotted curve, and finally converges to the approximate solution $G_{\theta^*}(z_{\text{new}}^*) = G_{\theta^*}(z_{\text{new}}^{(12)}) \approx G(\eta_{\text{new}})$.



\subsection{Meta-Auto-Decoder with Fine-Tuned Model}\label{sec:MAD_LM}

Assumption~\ref{as:lowdim} may fail in some cases, especially when the parameter set $\mathcal{A}$ of PDEs is an infinite-dimensional function space. 
In this case, we consider the following weaker assumption: 
\begin{assumption}\label{as:lowdimApprox}
	The solution set $G(\mathcal{A})\subset\mathcal{U}$ can be approximated by a set in a low-dimensional space if there is a finite-dimensional space $Z=\R^l$ (with $l\ll\dim\mathcal{U}$) and a Lipschitz continuous mapping $\bar G:Z\to\mathcal{U}$,
	such that $G(\mathcal{A})$ is contained in a $c$-neighborhood of $\bar G(Z)\subset\mathcal{U}$, where $c$ is a relatively small constant. 
	In other words, for any $\eta\in\mathcal{A}$, there exists some $z\in Z$ satisfying $\|\bar G(z)-G(\eta)\|_\mathcal{U}\le c$. 
\end{assumption}

% Appendix \ref{appendix:example_assumption2} gives an example of $G(\mathcal{A})$ which satisfies Assumption~\ref{as:lowdimApprox} but violates Assumption~\ref{as:lowdim}. 
Appendix A gives an example of $G(\mathcal{A})$ which satisfies Assumption~\ref{as:lowdimApprox} but violates Assumption~\ref{as:lowdim}. 
Under this new assumption, similar derivation leads to the same pre-training stage, and we use it to find the initial decoder mapping $G_{\theta^*}\approx\bar G$. 
However, in the fine-tuning stage, simply fine-tuning the latent vector $z$ won't give a satisfactory solution in general due to the existence of the $c$-gap. 
Therefore, we have to fine-tune the model weight $\theta$ with the latent vector $z$ simultaneously, and solve the following optimization problem
\vspace{-0.2cm}
\begin{equation}\label{eq:MADinf_LM}
	(z_{\text{new}}^*,\theta_{\text{new}}^*)=\operatorname*{\arg\min}_{z,\theta}\hat L^{\eta_{\text{new}}}[u(\cdot,z;{\theta})]+\frac1{\sigma^2}\|z\|^2
\end{equation}
with initial model weight $\theta^*$. 
It produces a new decoder $G_{\theta_{\text{new}}^*}(z_{\text{new}}^*)$ specific to the parameter $\eta_{\text{new}}$.

An intuitive illustration is given in Fig.\ref{fig:MADft} where the solution set $G_{\theta^*}(Z)$ obtained by the pre-training stage is represented by an orange solid curve, and the solution set $G(\mathcal{A})$ lies within a neighborhood of $G_{\theta^*}(Z)$ that is represented by a gray shadow band. 
To find solution $u^{\eta_{\text{new}}}$, we have to fine-tune $\theta$ (i.e., the orange dotted lines) and the latent vector $z$ (i.e., the points on the orange dotted line) simultaneously to approach the exact solution. 
As the search scope is limited to a strip with a small width, the fine-tuning process converges quickly.

% \begin{figure}
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{figures/method_ADintuition-ft.png}}
% \caption{
% 	Illustration of how MAD with fine-tuned model works from the manifold learning perspective. 
% }
% \label{fig:MADft}
% \end{center}
% \end{figure}

==> sections/related_work.tex <==
\section{Related work}\label{sec:related_work}
In this section, we review the learning-based PDE solvers and classify these solvers into two categories in terms of the objects that are approximated by neural networks (NN), i.e., the approximation of the solution and the approximation of the solution mapping.
In addition, we also briefly discuss the related meta-learning algorithms and the auto-decoder architecture.

\subsection{NN as a new ansatz of solution}
This kind of approaches approximate the solution of the PDEs with a neural network and mainly rely on governing equations and boundary conditions (or their variants) to train the neural networks. 
For example, PINNs \cite{raissi2018deep} and DGM \cite{sirignano2018dgm} constrain the output of deep neural networks to satisfy the given governing equations and boundary conditions. 
Deep Ritz Method (DRM) \cite{weinan2018deep} exploits the variational form of PDEs and can be used to solve PDEs that can be reformulated as equivalent energy minimization problems. 
Based on a weak formulation of PDEs, Weak Adversarial Network (WAN) \cite{zang2020weak} parameterizes the weak solution and test functions as primal and adversarial neural networks, respectively. 
These neural approximation methods can work in an unsupervised manner, without the need to generate labeled data from conventional computational methods. 
However, none of them can be used to solve parametric PDEs as they have to retrain the neural network under different PDE parameters.
In order to mitigate retraining cost, \citet{weinan2018deep} recommends a transfer learning method that uses a model trained for one task as the initial model to train another task. 
However, according to our experiments transfer learning method is not always effective in improving convergence speed (see Sec.\ref{sec:burgers} and Sec.\ref{sec:laplace}). 
% We consider this to be the phenomenon of negative transfer \cite{weiss2016survey}. 
% An important prerequisite of transfer learning is that the target task is similar to the source task, however, when the relationship between the two tasks is weak, negative transfer occurs.

\subsection{NN as a new ansatz of solution mapping}
This kind of approaches use neural networks to learn the solution mapping between two infinite-dimensional function spaces \cite{long2018pde,long2019pde,lu2019deeponet, bhattacharya2020model, li2020fourier}.
For example, PDE-Nets \cite{long2018pde,long2019pde} are among the earliest neural operators that are specifically designed convolutional neural networks inspired by finite difference approximations of PDEs. 
They are able to uncover hidden PDE models from observed dynamical data and perform fast and accurate  predictions at the same time.
DeepONet \cite{lu2019deeponet} uses two subnets to encode the parameters and location variables of the PDEs separately, and merge them together to compute the solution.
Fourier Neural Operator (FNO) \cite{li2020fourier} utilizes fast Fourier transform to build the neural operator architecture and learn the parameter-to-solution mapping between two infinite-dimensional function spaces.
A significant advantage of these approaches is that once the neural network is trained, the prediction time is almost negligible. 
However, the data acquisition cost is prohibitive in complex physical, biological, or engineering systems, and the generalization ability of these models is poor when there is no enough labeled data \cite{cai2021physics}.

\subsection{Meta-Learning}
As solving parametric PDEs can be viewed as a meta-learning problem, we investigate a class of meta-learning algorithms that include the original model-agnostic meta-learning (MAML) \cite{finn2017model} algorithm and its variants \cite{antoniou2019train, nichol2018reptile, yoon2018bayesian}. These algorithms try to find an initial model with good generalization ability such that it can be adapted to new tasks with a small number of gradient updates.  
For example, the model-agnostic meta learning (MAML) \cite{finn2017model} firstly trains a meta-model with good initialization weight on a variety of learning tasks, which is then fine-tuned on a new task through a few steps of gradient descent to get the target model.
The Reptile \cite{nichol2018reptile} algorithm eliminates second-order derivatives in MAML algorithm by repeatedly sampling a task, training on it, and moving the initialization towards the trained weight on that task.
Recently, Reptile algorithm is used to solve the PDE problems in \cite{liu2021novel}.
However, MAML and Reptile are not always effective in improving convergence speed (see Sec.\ref{sec:maxwell} and Sec.\ref{sec:laplace}), whereas our MAD method is effective in all cases. 

\subsection{Auto-Decoder}
\citet{park2019deepsdf} present an interesting work in 3D computer vision that can generate any 3D shape from a shape description. 
Each shape description is encoded as a latent vector, and an auto-decoder is constructed to represent the mapping from the latent space to a distribution of complex shapes. 
Different from an auto-encoder whose latent code is produced by the encoder, an auto-decoder directly accepts a latent vector as an input.
Unlike the auto-decoder in \cite{park2019deepsdf} which only refines the latent vector, MAD refines both latent vector and neural network's weight as originating naturally from the manifold learning understanding.






